Large-Scale Geometry of Pure Mapping Class Groups of Infinite-Type Surfaces

The work of Mann and Rafi gives a classification surfaces $\Sigma$ when $\textrm{Map}(\Sigma)$ is globally CB, locally CB, and CB generated under the technical assumption of tameness. In this article, we restrict our study to the pure mapping class group and give a complete classification without additional assumptions. In stark contrast with the rich class of examples of Mann--Rafi, we prove that $\textrm{PMap}(\Sigma)$ is globally CB if and only if $\Sigma$ is the Loch Ness monster surface, and locally CB or CB generated if and only if $\Sigma$ has finitely many ends and is not a Loch Ness monster surface with (nonzero) punctures.

==> cutthings.tex <==
For the remainder of this section, we will describe: 
\begin{enumerate}
    \item a proof sketch of Mann--Rafi's original argument rephrased for $\PMap(\S)$; 
    \item an alternative proof following {\cite[Theorem 3.9]{horbez2022big}} that uses the projection complexes introduced by Bestvina--Bromberg--Fujiwara (see \cite{bestvina2015constructing}). 
\end{enumerate}
Both methods aim to extend the unboundedness of the action of pseudo-Anosov elements on the curve complex of a finite-type subsurface proven by Masur--Minsky \cite{MR1714338}.  Curve graphs and subsurface projections will play a role in both proofs. 

\subsubsection{Proof Using Projection Complexes} 
This proof follows the strategy of {\cite[Theorem 3.9]{horbez2022big}}. 
Instead of building an unbounded length function, the idea is to disprove the CB-ness of $\PMap(\S)$ directly by constructing a metric space $X$ on which $\PMap(\S)$ acts with unbounded orbits.  
Like Mann--Rafi's proof, this strategy also applies to disprove the CB-ness of the full mapping class group in the presence of a nondisplaceable subsurface. 
However, we will phrase the proof in the context of $\PMap(\S)$ for our purpose.  

Projection complexes were first introduced in \cite{bestvina2015constructing}.   
To construct a projection complex, we need the following data: 
\begin{itemize}
    \item a collection of metric spaces $\Y = \set{X, Y, Z, \dots}$, 
    \item projection functions $\pi_Y \colon \Y \setminus \set{Y} \to Y$. 
\end{itemize}
The projection distance is defined as $d_Y(X, Z) \dfn \operatorname{diam}_Y (\pi_Y(X) \cup \pi_Y(Z))$ and we require that $(\Y, \set{\pi_Y})$ satisfy the following projection axioms for some projection constant $\theta \ge 0$ and all $X, Y, Z \in \Y$ distinct: 
\begin{itemize}
    \item[(P1)] $\operatorname{diam}(\pi_X(Y)) \le \theta$;
    \item[(P2)] (Behrstock Inequality) If $d_X(Y, Z) > \theta$, then $d_Y(X,Z) \le \theta$ and $d_Z(X,Y) \le \theta$; i.e. only one of the projections can be large.  This gives a notion of ``in-between-ness'';  
    \item[(P3)] The set $\set{Z \in \Y \mid d_Z(X,Y) > \theta}$ is finite; i.e., there are only finitely many spaces between  $X$ and $Y$.  
\end{itemize}
For some $K \ge 0$, the \textbf{projection complex} denoted by $P(\Y, \theta, K)$ is a graph whose vertices are the elements of $\Y$ where vertices $X$ and $Z$ are connected by an edge if $d_Y(X, Z) \le K$ for all $Y \in \Y\setminus\set{X,Z}$.
%\THcomment{Ask Sanghoon if this extra condition corrects this statement...}
%\SKcomment{Hmm what I intended to point out was that you used the `in-between' analogy for $\theta$ already, so it might not be clear to use the same analogy for $K$ possibly larger than $\theta$.}

We can also define the \textbf{quasi-tree of spaces} or \textbf{blown up projection complex}, denoted by $\C(\Y, \theta, K)$, by connecting the metric spaces $Z$ and $X$ with arcs between $\pi_Z(X)$ and $\pi_X(Z)$ if and only if $d_Y(X,Z) \le K$ for all $Y \in \Y \setminus \set{X,Z}$.  

\begin{FACT}
    [{\cite[Section 4.4]{bestvina2015constructing}} ]
    \label{fact:projaction}
    If $G$ acts on $\bigsqcup_{X \in \Y} X$ by isometries, permuting the spaces, and commuting with the projections i.e. $g(\pi_X(Y)) = \pi_{g(X)}(g(Y))$, then the action of $G$ extends to actions on $P(\Y, \theta, K)$ and $\C(\Y, \theta, K)$ by isometries.  
\end{FACT}

With this generic setup, we now focus on our setting.  Recall that $S$ is a nondisplaceable subsurface in $\S$, and $\mathcal{C}(Y)$ denotes the curve graph of a subsurface $Y \subset \S$.  

\begin{FACT}
    [{\cite[Section 5]{bestvina2015constructing} }] 
    \label{fact:ProjCompSurf}
    Let $\mathcal{I} = \set{f(S) \mid f \in \PMap(\S)}$, $\Y = \set{\C(Y) \mid Y \in \mathcal{I}}$, and $\pi_Y \colon \Y \setminus \C(Y) \to \C(Y)$ be the subsurface projection.  Then for some $K, \theta \ge 0$, $(\Y, \set{\pi_Y}, K, \theta)$ satisfies the projection axioms.  
\end{FACT}

While \Cref{fact:ProjCompSurf} is phrased in the context of finite-type surfaces, this also holds true for infinite-type surfaces. 
\Thomas{add explanation here} 
Thus from $(\Y, \set{\pi_Y}, K, \theta)$ we can build the blown up projection complex $\C_K(\Y) = \C(\Y, K, \theta)$.   Because the action of $\PMap(\S)$ on $(\Y, \set{\pi_Y})$ satisfies the hypothesis of \Cref{fact:projaction}, $\PMap(\S)$ acts on $\C_K(\Y)$ by isometries.  

\begin{proof}[Proof of \Cref{prop:nondisp}]
Finally, as in the previous proof, we pick $\phi \in \PMap(\S)$ that preserves $S$ and $\phi_{|S}$ is a pseudo-Anosov.  Then $\phi$ has infinite translation length on the curve graph of $S$, so $d_S(\gamma, \phi^n(\gamma)) \to \infty$ as $n \to \infty$ for every essential simple closed curve $\gamma$ by \cite{MR1714338}.  Since $\C(S)$ is quasi-isometrically embedded in $\C_K(\Y)$ 
\Thomas{insert reference to \cite{bestvina2015constructing} look for the right proposition...}
, it follows that $d_{\C_K(\Y)}(\gamma, \phi^n(\gamma)) \to \infty$ as $n \to \infty$.  Thus the action of $\PMap(\S)$ on $\C_K(\Y)$ has unbounded orbit $\PMap(\S) \cdot [\gamma]$, and therefore $\PMap(\S)$ is not CB.  
\end{proof}



\begin{LEM}\Priyam{add that $\S$ is infinite-type to statement of Lemma. Check that you don't drop this quantifier in other statements}
    \label{lem:oneIsolatedPunct} A \textbf{puncture} is an isolated planar end. 
    If $\S$ has a puncture, $\S$ has a nondisplaceable subsurface with respect to $\PMap(\S)$.
\end{LEM}

\begin{proof}
    \Priyam{I think you want to break this into cases in a different way that leads to an easier proof: the surface has infinitely many punctures or finitely many punctures. If infinitely many then ends $\geq 3$ and you are done. If finitely many punctures, then take the surface containing those finitely many punctures and it's nondispaceable wrt the *full* mapping class group and so also for the pure} \Priyam{looking over your argument below again, I don't even think you need to write out this lemma. You only use it for the case of the once punctures loch ness which can easily be seen to have a non-disp subsurface, containing the one punture.}
    If $\S$ has zero or finitely many genus, then for it to be infinite-type it must have infinitely many punctures in which case $|E(\S)| \ge 3$ and \Cref{lem:threeEnds} guarantees $\S$ has a nondisplaceable subsurface with respect to $\PMap(\S)$. 

    Otherwise, if $\S$ has infinite genus, then the subsurface $K$ homeomorphic to a torus with two boundary components  pictured below in \Cref{pic:isolatedpuncture} is nondisplaceable.

    \begin{figure}[ht!]
    \centering
    \begin{overpic}[width=4cm]{isolatedpunct.jpeg}
        \put(32,34){\color{blue} $K$}
        \put(10,18){$S_0$}
        \put(65,10){$S_1$}
    \end{overpic}
    \caption{The subsurface $K$ is nondisplaceable with respect to $\PMap(\S)$. 
    \label{pic:isolatedpuncture}
    }
\end{figure}

    
    
    The proof that $K$ is nondisplaceable follows a similar strategy as the proof of \Cref{lem:threeEnds}.  Let $\S \setminus K = S_0 \sqcup S_1$ where $E(S_0) = \set{p}$ is a puncture. 
    If $K$ were displaceable, then for some $f \in \PMap(\S)$ we would have $f(K) \cap K = \emptyset$.  Because $K$ has genus and $S_0$ does not, $f(K) \subset S_1$.  Let $\S \setminus f(K) = S_0' \sqcup S_1'$ where up to relabeling $S_i' \cong S_i$.   
    Because $K \cup S_0$ is connected and disjoint from $f(K)$, $K\cup S_0$ lies completely in one of the $S_i'$, but since $K \cup S_0$ has 1 genus and $S_0' \cong S_0$ does not, it must be that $S_0 \cup K \subset S_1'$. 
    This means that $\set{p} = E(S_0) \subset E(S_1')$ which is a contradiction since $E(S_1') = E(S_1)$ by \Cref{eqn:HomEnds} in \Cref{lem:threeEnds}, but $E(S_0) \cap E(S_1) = \emptyset$. 
\end{proof}

Specifically, a surface $\S$ is called \textbf{telescoping} \Priyam{do you ever use this definition of telescoping? If not I would delete it.} if there exist a pair of ends $x_1,x_2 \in E(\S)$ and disjoint clopen neighborhoods $V_1, V_2$ of $x_1, x_2$ respectively, such that for every clopen sub-neighborhood $W_i \subset V_i$ of $x_i$, there are homeomorphisms $f_1, f_2$ 
(called big zoom) 
and $h_1, h_2$ 
(called little zoom) 
of $\S$ all fixing $x_1$ and $x_2$ where 
\begin{align*}
    f_1(W_1) &\supset \S - V_2, \qquad h_1(W_1) = V_1, \qquad \text{and } \quad h_1(V_2) = V_2,\\
   f_2(W_2) &\supset \S - V_1, \qquad h_2(W_2) = V_2, \qquad \text{and } \quad h_2(V_1) = V_1.
\end{align*}


%Proof of lemma 3.3 

Recall that 
\begin{equation*} 
    1 \to \PMap(\S) \to \Mp(\S) \xrightarrow{\phi} \Homeo(E(\S), E_G(\S)) \to 1 
    \end{equation*} 
    and when $|E(\S)|< \infty$, $\Homeo(E(\S), E_G(\S))$ is a finite group, specifically $\Sym(n) \times \Sym(m)$ where $n$ is the number of punctures, and $m$ is the number of ends accumulated by genus. By exactness of the sequence, 
    \begin{equation*} 
    \Sym(n) \times \Sym (m) \cong \Mp(\S)/\ker(\phi) \cong \Mp(\S)/\PMap(\S)  
    \end{equation*} 
    hence $\PMap(\S)$ has finite index in $\Mp(\S)$.  
    Because $\Mp(\S)$ is a Polish group and $\PMap(\S)$ is a clopen Polish subgroup, the desired result follows from \Cref{fact:CEmbed}.    



    \begin{RMK}
    \label{rmk:SSTelEndsInf}
    A telescoping surface necessarily has infinitely many ends (see {\cite[Proposition 3.7]{mann2019large}}).
    Likewise, self-similar end spaces contain either a single end or infinitely many ends. 
    \textcolor{magenta}{To see this, note that if $E(\S)$ were self-similar with $1 < |E(\S)|< \infty$, then for the partition of the end space into singleton sets $E(\S) = \set{x_1} \sqcup \dots \sqcup \set{x_n}$ we must have some $D \subset \set{x_i}$ such that $(D, D\cap E_G(\S)) \cong (E(\S), E_G(\S))$, but $|D| \ne |E(\S)|$ as finite sets, so this is not possible. } 
\end{RMK}

%\begin{EX} 
%    There are examples of surfaces whose end space is self-similar but not telescoping and vice versa, as well as surfaces that are both.  For instance, the Cantor tree surface is self similar and telescoping.  
%    The Cantor tree surface with one end accumulated by genus is self-similar, but not telescoping. 
 %   A surface with $E_G(\S)$ a Cantor set and total end space $E(\S)$ the union of $E_G(\S)$ and another Cantor set set intersecting $E_G(\S) $ in two points is an example of a surface with telescoping, but not self-similar end space.
%\end{EX}

\textcolor{magenta}{The definition of the tameness condition mentioned in \Cref{fact:MRgloballyCB} relies on the partial order on the set of ends. 
For distinct $x, y \in E(\S)$, we say that $y \preccurlyeq x$ if for any neighborhood $U$ of $x$, there is a neighborhood $V$ of $y$ and $f \in \Mp(\S)$ such that $f(V) \subseteq U$.  An end $x$ is \textbf{maximal} if $x \preccurlyeq y$ implies $x \sim y$. Mann--Rafi prove that maximal ends exist with respect to the partial order, the set of maximal ends $\mathcal{M}(E(\S))$ is non-empty, and is either finite or a Cantor set (see {\cite[Proposition 4.7]{mann2019large} }). An \textbf{immediate predecessor} of a maximal end $x$ is an end $y$ with $y \prec x$, such that there are no ends $z$ for which $y \prec z \prec x.$}

\textcolor{magenta}{While this partial order is an important tool in understanding the classification of surfaces with locally CB and CB-generated mapping class groups, the partial order is not meaningful the context of the \emph{pure} mapping class group since all ends become incomparable under this restriction.  To see why, suppose that $y \preccurlyeq x$.  Then for any neighborhood $U$ of $x$, there is a mapping class $f$ and a neighborhood $V$ of $y$ so that $f(V) \subset U$. In particular, this holds for a neighborhood $U$ of $x$ that is disjoint from $y$.  But this means $f(y) \in U$, while $y \not\in U$ so $f$ cannot have been a pure mapping class. }
 
\textcolor{magenta}{
\begin{DEF} 
    An end $e$ is called \textbf{stable} if it is ``locally self-similar'', that is if there is a neighborhood $U$ of $e$ such that all sub-neighborhoods $U'$ of $e$ contain a homeomorphic copy of $U$.   
    An end space is \textbf{tame} if 
    \begin{itemize}
        \item all maximal ends are stable,
        \item all immediate predecessors of maximal ends are stable. 
    \end{itemize}
\end{DEF}}


\begin{RMK}
    \label{rmk:finTame}
    If $|E(\S)| < \infty$, then $\S$ is tame. \textcolor{magenta}{To see why, it suffices to check that all ends $x \in E(\S)$ are stable.  Since $|E(\S)| < \infty$, all ends are isolated. Because of this, we can find a small enough neighborhood $U$ about the end $x$ so that $E(U) = \set{x}$.  Then any sub-neighborhood $U' \subset U$ is homeomorphic to $U$ by the classification of surfaces, hence $x$ is stable and $\S$ is tame.  
\end{RMK}}



\begin{LEM}
    \label{lem:CoarselyEmbedded}
    If $|E(\S)| < \infty$, then $\PMap(\S)$ is CB if and only if $\Mp(\S)$ is CB. Furthermore, a subset $X \subset \PMap(\S)$ is CB in $\PMap(\S)$ if and only if $X \subset \Mp(\S)$ is CB in $\Mp(\S)$. 
    \Priyam{do you need the second sentence? I think you do for locally CB but the writing to the end of this subsection seems a bit out of order, let's talk about it together. Also, it seems like the main point of this lemma is to say that when ends are finite, Pmap is finite index in Map. This is widely known so I don't think you need to prove it. Instead you can just say that and that Pmap is clopen and then say that this means Fact 2.6 kicks in.} 
    \Thomas{We will use the second part of the sentence for the locally CB classification. I re-wrote the proof to omit the proof that $\PMap(\S)$ is finite index in $\Mp(\S)$.  }
\end{LEM}

\begin{proof}
When $|E(\S)|< \infty$ recall that $\PMap(\S)$ has finite index in $\Mp(\S)$. Because $\Mp(\S)$ is a Polish group and $\PMap(\S)$ is a clopen Polish subgroup, the desired result follows from \Cref{fact:CEmbed}.  
\end{proof} 
